Globular Cluster Abundances from High-Resolution Integrated Light Spectra, I: 47 Tuc

We describe the detailed chemical abundance analysis of a high-resolution (R~35,000), integrated-light (IL), spectrum of the core of the Galactic globular cluster 47 Tuc, obtained using the du Pont echelle at Las Campanas. We develop an abundance analysis strategy that can be applied to spatial unresolved extra- galactic clusters. We have computed abundances for Na, Mg, Al, Si, Ca, Sc, Ti, V, Cr, Mn, Fe, Co, Ni, Cu, Y, Zr, Ba, La, Nd and Eu. For an analysis with the known color-magnitude diagram (cmd) for 47 Tuc we obtain a mean [Fe/H] value of -0.75 +/-0.026+/-0.045 dex (random and systematic error), in good agreement with the mean of 5 recent high resolution abundance studies, at -0.70 dex. Typical random errors on our mean [X/Fe] ratios are 0.07-0.10 dex, similar to studies of individual stars in 47 Tuc, although Na and Al appear enhanced, perhaps due to proton burning in the most luminous cluster stars. Our IL abundance analysis with an unknown cmd employed theoretical Teramo isochrones; however, we apply zero-point abundance corrections to account for the factor of 3 underprediction of stars at the AGB bump luminosity. While line diagnostics alone provide only mild constraints on the cluster age (ruling-out ages younger than ~2 Gyr), when theoretical IL B-V colors are combined with metallicity derived from the Fe I lines, the age is constrained to 10--15 Gyr and we obtain [Fe/H]=-0.70 +/-0.021 +/-0.052 dex. We find that Fe I line diagnostics may also be used to constrain the horizontal branch morphology of an unresolved cluster. Lastly, our spectrum synthesis of 5.4 million TiO lines indicates that the 7300-7600A TiO window should be useful for estimating the effect of M giants on the IL abundances, and important for clusters more metal-rich than 47 Tuc.

==> bibliography.tex <==
\begin{thebibliography}{}

\bibitem[Alonso et al.~(1999)]{a99}
Alonso, A., Arribas, S. \& Martinez-Roger, C. 1999, A\&AS, 140, 261
%``The Effective Temperature Scale of Giant Stars (F0--K5). II. Empirical
% Calibration of T$_{\rm eff}$ Verses Colours and [Fe/H]"

\bibitem[Alonso et al.~(2001)]{a01}
Alonso, A., Arribas, S. \& Martinez-Roger, C. 2001, A\&AS, 376, 1039
%``Erratum: The Effective Temperature Scale of Giant Stars (F0--K5). II. Empirical
% Calibration of T$_{\rm eff}$ Verses Colours and [Fe/H]"


\bibitem[Alves-Brito et al.~(2005)]{a05_01}
Alves-Brito, A., Barbuy, B., Ortolani, S., Momany, Y., Hill, V., Zoccali, M., Renzini, A. et al. 
2005, A\&A, 435, 657

\bibitem[Asplund et al.~(2005)]{a05_02}
Asplund, M., Grevesse, N. \& Sauval, A.J. 2005,
``Cosmic Abundances as Records of Stellar Evolution and Nucleosynthesis'', ASP Conference Series vol. 336, 2005, p.~25;
Austin, Texas; eds. F.N. Bash \& T.G. Barnes (also astro-ph/0410214).


\bibitem[Bai et al. (2004)]{1704}
Bai, G.S., Zhao, G., Chen, Y.Q., Shi, J.R., Klochkova, V.G., Panchuk, V.E., Qui, H.M., \&
Zhang, H.W. 2004, A\&A 425, 671

\bibitem[Bernstein \& McWilliam (2005)]{bm05}
Bernstein, R.A., \& McWilliam, A. 2005, in ``Resolved Stellar Populations'', ASP Conf Series,
                 eds. D. Valls-Gabaud and M. Chavez  (astro-ph/0507042)

\bibitem[Brodie \& Huchra (1990)]{bh90}
Brodie, J.P., \& Huchra, J.P. 1990, ApJ, 362, 503

\bibitem[Brown et al. (1994)]{bsl94}
Briley, M.M., Smith, V.V., \& Lambert, D.L. 1994, ApJ, 424, L119

\bibitem[Brown \& Wallerstein (1992)]{bw92}
Brown, J.A., \& Wallerstein, G. 1992, AJ, 104, 1818

\bibitem[Carretta et al.~2004]{cg47t}
Carretta, E., Gratton, R.G., Bragaglia, A., Bonifacio, P., \& Pasquini, L. 2004, A\&A, 416, 925

\bibitem[Cohen 1978]{cohen78}
Cohen, J.G., 1978, ApJ, 223, 487

\bibitem[Cassisi \& Salaris 1997]{cs97}
Cassisi, S., \& Salaris, M. 1997, \mnras, 285, 593

\bibitem[Cassisi, Salaris & Irwin 2003]{1727}
Cassisi, S., Salaris, M. \& Irwin, A.W. 2003, ApJ, 588, 862

\bibitem[Castelli \& Kurucz~2004]{1730}
Castelli, F., \& Kurucz, R.L. 2004, IAU Symposium 210, ``Modelling of Stellar Atmospheres'',
eds. N. Piskanov et al., poster A20 (astro-ph/0405087)

\bibitem[Castilho et al.~2000]{castilho}
Castilho, B.V., Pasquini, L., Allen, D.M., Barbuy, B., \& Molaro, P. 2000, A\&A, 361, 92

\bibitem[Edvardsson (1993)]{1737}
Edvardsson, B., Andersen, J., Gustafsson, B., Lambert, D.L., Nissen, P.E., \& Tomkin, J.
    1993, \aap, 275, 101

\bibitem[Elson \& Santiago (1996)]{1741}
Elson R.A.W., \& Santiago, B.X. 1996, \mnras, 278, 617

\bibitem[Faber (1973)]{1744}
Faber, S.M. 1973, ApJ, 179, 731

\bibitem[Faber~\&~Jackson~(1976)]{1747}
Faber, S.M., \& Jackson R.E. 1976, ApJ, 204, 668

\bibitem[Faber et al.~(1985)]{faber85}
Faber, S.M., Friel, E.D., Burstein, D.,, \& Gaskell, C.M. 1985, ApJS, 57, 711

\bibitem[Forte, Strom \& Strom 1981]{fss81}
Forte, J.C., Strom, S.W., \& Strom, K.M. 1981, ApJ, 245, L9

\bibitem[Ferguson et al. 2005]{1756}
Ferguson, J.W., Alexander, D.R., Allard, F., Barman, T., Bodnarik, J.G., Hauschildt, P.H., Heffner-Wong, A., Tamanai, A.
2005, ApJ, 623, 585.


\bibitem[Ferraro et al. 1997]{1761}
Ferraro, F.R., Carretta, E., Bragaglia, A., Renzini, A., Ortolani, S.

\bibitem[Fulbright, McWilliam \& Rich 2006]{fmr06}
Fulbright, J., McWilliam, A., \& Rich, R.M. 2006, ApJ, 636, 821

\bibitem[Geisler et al. 1996]{g96}
Geisler, D., Lee, M.G., \& Kim, E. 1996, AJ, 111, 1529

\bibitem[Girardi et al. 2000]{1770}
Girardi et al. 2000, AAS 141, 371

\bibitem[Gouliermis et al. 2004]{1773}
Gouliermis, D., Keller, S.C., Kontizas, M., Kontizas, E., Bellas-Velidis, I. 2004, A\&A, 416, 137

\bibitem[Salasnich et al. 2000]{1776}
Salasnich et al. 2000, AA 361, 1023

\bibitem[Gratton et al. 1994]{1779}
Gratton, R.G. \& Sneden, C. 1994, \aap, 287, 927

\bibitem[Gratton et al. 2003]{1782}
Gratton, R.G., Bragaglia, A., Carretta, E., Clementini, G., Desider, S., Grundahl, F., \&
       Lucatello, S. 2003, AA, 408, 529

\bibitem[Grevesse \& Sauval (1999)]{1786}
Grevesse, N., \& Sauval, A.J. 1999, A\&A, 347, 348

\bibitem[Guhathakurta et al. 1992]{1789}
Guhathakurta, P., Yanny, B., Schneider, D.P., \& Bahcall, J.N. 1992, AJ, 104, 1790

\bibitem[Harris 1991]{1792}
Harris, W.E. 1991, ARA\&A, 29, 543

\bibitem[Houdashelt et al. 2000]{1795}
Houdashelt, M.L., Bell, R.A., Sweigart, A.V., \& Wing, R.F. 2000, ApJ, 119, 1424

\bibitem[Howell et al. 2000]{1798}
Howell, J.H., Guhathakurta, P., \& Gilliland, R.L. 2000, PASP, 112, 1200

\bibitem[Johnson 2002]{1801}
Johnson, J.A. 2002, ApJS, 139, 219

\bibitem[Kaluzny 1997]{1804}                 
Kaluzny, J. 1997, A\&AS, 122, 1

\bibitem[Kaluzny et al. 1998]{1807}                 
Kaluzny, J., Kubiak, M., Szymanski, M., Udalski, A., Krzeminski, W., Mateo, M. \& Stanek, K.Z.
        1998, A\&AS, 128, 19

\bibitem[Kaufer et al.~2004]{1811}                   
Kaufer, A., Venn, K.A., Tolstoy, E., Pinte, C., Kudritzki, R.P. 2004, AJ, 127, 2723

\bibitem[King et al.~1995]{1814}                   
King, I.R., Sosin, C., \& Cool, A.M. 1995, ApJ, 452, L36

\bibitem[Koch \& McWilliam (2008)]{1817}                   
Koch, A., \& McWilliam, A. 2007, in preparation

\bibitem[Kroupa~2002]{1820}                   
Kroupa, P., 2002, Science, 295, 82

\bibitem[Ku\check{c}inskas et al.~2006]{1823}                   
Ku$\check{c}$inskas, A., Hauschildt, P.H., Brott, I., Vansevi$\check{c}$ius, V., Lindegren, L., Tanab$\acute{e}$, T., 
\& Allard, F. 2006, A\&A, 452, 1021

\bibitem[Letarte et al. 2006]{let06}                   
Letarte, B., Hill, V., Jablonka, P., Tolstoy, E., Francois, P., \& Meylan, G. 2006, A\&A, 453, 547

\bibitem[Lebzelter \& Wood 2005]{1830}                   
Lebzelter, T. \& Wood, P.R. 2005, A\&A, 441, 1117

\bibitem[Luck \& Bond (1985)]{lb85}
Luck, R.E., \& Bond, H.E. 1985, ApJ, 292, 559

\bibitem[Maraston 2005]{1836}
Maraston, C. 2005, MNRAS, 362, 799

\bibitem[Maraston et al. 2006]{1839}
Maraston, C., Daddi, E., Renzini, A., Cimatti, A., Dickinson, M., Papovich, C., 
           Pasquali, A., \&  Pirzcal, N. 2006, ApJ, 652, 85

\bibitem[McWilliam 1997]{1843}
McWilliam, A. 1997, ARAA, 35, 503

\bibitem[McWilliam \& Bernstein 2002]{1846}
McWilliam, A., \& Bernstein, R.A. 2002, in ``Extragalactic Star Clusters'', IAU Symposium 207,
       Held in Pucon, Chile March 12-16, 2001. 
       Edited by D. Geisler, E.K. Grebel, and D. Minniti.
       San Francisco: Astronomical Society of the Pacific, 2002., p.739

\bibitem[McWilliam, Rich \& Smecker Hane 2003]{1852}
McWilliam, A., Rich, R.M., Smecker Hane, T.A. 2003, ApJ, 592, L21

\bibitem[Mishenina et al. 2002]{1855}
Mishenina, T.V., Kovtyukh, V.V., Soubiran, C., Travaglio, C., \& Busso, M. 2002, 
A\&A, 396, 189

\bibitem[Nissen et al. (2000)]{1859}
Nissen, P.E., Chen, Y.Q., Schuster, W.J., \& Zhao, G. 2000, A\&A, 353, 722

\bibitem[Paresce et al. 1995]{1862}
Paresce, F., de Marchi, G., Jedrzejewski, R. 1995, ApJ, 442, L57

\bibitem[Peng, Ford \& Freeman (2004)]{1865}
Peng, E.W., Ford, H.C., \& Freeman, K.C. 2004, \apj, 602, 705

\bibitem[Peterson (1986)]{peterson86}
Peterson, C.J. 1986, \pasp, 98, 192

\bibitem[Pietrinferni et al. (2006)]{1868}
Pietrinferni, A., Cassisi, S., Salaris, M., \& Castelli, F. 2006,  ApJ, 642, 797

\bibitem[Pilachowski et al. 1980]{p80}
Pilachowski, C.A., Canterna, R., \& Wallerstein, G. 1980, ApJ, 235, L21

\bibitem[Plez 1998]{1874}
Plez, B. 1998, A\&A, 337, 495

\bibitem[Prochaska \& McWilliam (2000)]{1877}
Prochaska, J.X., \& McWilliam, A. 2000, ApJ, 537, 57


\bibitem[Pryor \& Meylan 1993]{1881}
Pryor, C. \& Meylan, G. 1993, ASP Conference Series, vol. 50, 357.
             S.G. Djorgovski and G. Meylan (eds.)


\bibitem[Racine, Oke \& Searle 1978]{1886}
Raceine, R., Oke, J.B., \& Searle, L. 1978, ApJ, 223, 82

\bibitem[Schiavon et al. 2002]{1889}
Schiavon, R.P., Faber, S.M., Rose, J.A., \& Castilho, B.V. 2002, ApJ, 580, 873

\bibitem[Schlegel et al. 1998]{1892}
Schlegel, D.J., Finkbeiner, D.P., \& Davis, M. 1998, ApJ, 500, 525

\bibitem[Simmerer et al.(2003)]{1895}
Simmerer, J., Sneden, C., Ivans, I.I., Kraft, R.P., Shetrone, M.D., \& 
Smith, V.V. 2003, AJ, 125, 2018

\bibitem[Smith \& Lambert (1985)]{1899}
Smith, V.V. \& Lambert, D.L., 1985, ApJ, 294, 326

\bibitem[Sneden, C. 1973]{1902}
Sneden, C. 1973, ApJ, 184, 839

\bibitem[Sneden et al. 1973]{s91}
Sneden, C., Kraft, R.P., Prosser, C.F., \& Langer, G.E. 1991, AJ, 102, 2001

\bibitem[Sobeck et al. 2006]{1908}
Sobeck, J.S., Ivans, I.I., Simmerer, J.A., Sneden, C., Hoeflich, P., Fulbright, 
J.P., \& Kraft, R.P. 2006, ApJ, 131, 2949

\bibitem[Trager 2004]{1912}                   
Trager, S.C. 2004, in {\em Origin and Evolution of the Elements}, Carnegie Observatories 
                 Centennial Symposia, vol. 4. Cambridge University Press. 
                 Edited by A. McWilliam and M. Rauch, 2004, p. 391.


\bibitem[Venn et al.~2001]{1918}                   
Venn, K.A., Lennon, D.J., Kaufer, A., McCarthy, J.K., Przybilla, N., Kudritzki, R.P.,
Lemke, M., Skillman, E.D., \& Smartt, S.J. 2001, ApJ, 547, 765


\bibitem[Wallerstein 1962]{w62}                   
Wallerstein, G. 1962, ApJS, 6, 407

\bibitem[Whitmore et al. 1995]{1926}                   
Whitmore, B.C., Sparks, W.B., Lucas, R.A., Macchetto, F.D., \& Biretta, J.A. 1995, \apj, 454, L73

\bibitem[Winkler 1997]{1929}                   
Winkler, 1997, MNRAS, 287, 481

\bibitem[Worthey et al.~(1994)]{worthey94}
Worthey, G., Faber, S.M., Gonzalez, J.J., \& Burstein D. 1994, ApJS, 94, 687

\bibitem[Wylie et al. (2006)]{1935}                   
Wylie, E.C., Cottrell, P.L., Sneden, C.A., \& Lattanzio, J.C. 2006, ApJ, 649, 248

\bibitem[Zinn (1985)]{1938}                   
Zinn, R. 1985, ApJ, 293, 424

\end{thebibliography}

